Sequential Relaxation of Unit Commitment with AC Transmission Constraints

This paper proposes a sequential convex relaxation method for obtaining feasible and near-globally optimal solutions for unit commitment (UC) with AC transmission constraints. First, we develop a second-order cone programming (SOCP) relaxation for AC unit commitment. To ensure that the resulting solutions are feasible for the original non-convex problem, we incorporate penalty terms into the objective of the proposed SOCP relaxation. We generalize our penalization method to a sequential algorithm which starts from an initial point (not necessarily feasible) and leads to feasible and near-optimal solutions for AC unit commitment. Once a feasible point is attained, the algorithm preserves feasibility and improves the objective value until a near optimal point is obtained. The experimental results on IEEE 57, IEEE 118, and IEEE 300 bus benchmark cases from MATPOWER demonstrate the performance of the proposed method in solving challenging instances of AC unit commitment.

==> fig_1.tex <==
%%%%%%%%% ABSTRACT
\tikzset{
    master/.style={
        execute at end picture={
            \coordinate (lower right) at (current bounding box.south east);
            \coordinate (upper left) at (current bounding box.north west);
        }
    },
    slave/.style={
        execute at end picture={
            \pgfresetboundingbox
            \path (upper left) rectangle (lower right);
        }
    }
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\captionsetup[subfigure]{position=b}
\centering
\begin{tikzpicture}[master,scale=0.85]
\centering
\begin{axis}[
		width = 0.52\textwidth,
		height = 0.29\textwidth,
        xmode= normal,
		ymode= normal,	
    	ylabel= {$g(\cbf)$},
    	ylabel shift= -0.2cm,
%  		xmin= 0,
%   	xmax= 14000,
%       ymax= 0.1,
        xtick= \empty,
%       xshift = -1mm,
    	grid style = dashed,
        legend pos = north east,
		legend cell align = {left},
        legend image post style = {scale=0.7},
        legend style={font=\scriptsize, inner xsep=0.2pt, inner ysep=0.1pt},
]
% \draw[<->, densely dotted, line width= 0.05cm, Fcolor] (axis cs:400,0.003)--(axis cs:13750,0.003) node [black, pos=0.55, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{$\Wbf\!=\!\vbf\vbf^{\ast}$}};
% \draw[<->, densely dotted, line width= 0.05cm, Fcolor] (axis cs:1250,0.0056)--(axis cs:13750,0.0056) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{$\Wbf\!=\!\vbf\vbf^{\ast}$}};
% \draw[<->, densely dotted, line width= 0.05cm, Fcolor] (axis cs:6400,0.01)--(axis cs:13750,0.01) node [black, pos=0.5, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{$\Wbf\!=\!\vbf\vbf^{\ast}$}};
\addplot[dashed,color=blue,line width=0.5mm] table[x=iter,y=objective,col sep=comma] {57.csv};
% \legend{$\mathrm{SOCP}$}
\end{axis}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{0.1cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}[slave,scale=0.85]
\centering
\begin{axis}[
		width = 0.52\textwidth,
		height = 0.29\textwidth,
        xmode=normal,
		ymode=normal,	
      	ylabel= {$g(\cbf)$},
		ylabel shift = -0.1cm,
        xtick= \empty,
%   	xmin = 0,
%  		xmax = 14000,
%       xtickmax = 13000,
%       ymin = 14700,
%         xtick scale label code/.code={\pgfmathparse{int(#1)}$\mu \cdot 10^{\pgfmathresult}$},
%  		every x tick scale label/.style={at={(xticklabel cs:0.5)}, anchor = north},
%         ytick scale label code/.code={\pgfmathparse{int(#1)}$\text{Cost}\, \cdot 10^{\pgfmathresult}$},
%         every y tick scale label/.style={at={(yticklabel cs:0.5)}, anchor = south, rotate = 90},  
    	legend pos=south east,
    	grid style=dashed,
		legend cell align={left},
        legend image post style={scale=0.7},
        legend style={font=\scriptsize, inner xsep=0.2pt, inner ysep=0.1pt},
]
% \draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:400,16675)--(axis cs:13750,16675) node [black, pos=0.6, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{$\Wbf\!=\!\vbf\vbf^{\ast}$}};
% \draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:1250,17305)--(axis cs:13750,17305) node [black, pos=0.6, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{$\Wbf\!=\!\vbf\vbf^{\ast}$}};
% \draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:6400,18010)--(axis cs:13750,18010) node [black, pos=0.53, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{$\Wbf\!=\!\vbf\vbf^{\ast}$}};
\addplot[dashed,color=blue,line width=0.5mm] table[x=iter,y=objective,col sep=comma] {118.csv};

% \legend{$\mathrm{SOCP}$}
\end{axis}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{0.1cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tikzpicture}[slave,scale=0.85]
\centering
\begin{axis}[
		width = 0.52\textwidth,
		height = 0.29\textwidth,
        xmode=normal,
		ymode=normal,	
		ylabel shift = -0.1cm,
        ylabel= {$g(\cbf)$},
%   	xmin = 0,
%  		xmax = 14000,
%       xtickmax = 13000,
%       ymin = 14700,
%         xtick scale label code/.code={\pgfmathparse{int(#1)}$\mu \cdot 10^{\pgfmathresult}$},
%  		every x tick scale label/.style={at={(xticklabel cs:0.5)}, anchor = north},
%         ytick scale label code/.code={\pgfmathparse{int(#1)}$\text{Cost}\, \cdot 10^{\pgfmathresult}$},
%         every y tick scale label/.style={at={(yticklabel cs:0.5)}, anchor = south, rotate = 90},  
    	legend pos=south east,
    	grid style=dashed,
		legend cell align={left},
        legend image post style={scale=0.7},
        legend style={font=\scriptsize, inner xsep=0.2pt, inner ysep=0.1pt},
]
% \draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:400,16675)--(axis cs:13750,16675) node [black, pos=0.6, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{$\Wbf\!=\!\vbf\vbf^{\ast}$}};
% \draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:1250,17305)--(axis cs:13750,17305) node [black, pos=0.6, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{$\Wbf\!=\!\vbf\vbf^{\ast}$}};
% \draw[<->, densely dotted, line width= 0.06cm, Fcolor] (axis cs:6400,18010)--(axis cs:13750,18010) node [black, pos=0.53, above] {\footnotesize \raisebox{-0.2ex}[0pt][-0.2ex]{$\Wbf\!=\!\vbf\vbf^{\ast}$}};
\addplot[dashed,color=blue,line width=0.5mm] table[x=iter,y=objective,col sep=comma] {300.csv};

% \legend{$\mathrm{SOCP}$}
\end{axis}
\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{8mm}
\caption{Behavior analysis of the penalized relaxations for different choices of $\mu$.Top: feasibility violation; Bottom: total generation cost}
\vspace{-0.5mm}
\label{plt:plot_feas_cost}
\end{figure}

